Prediction of Object Geometry from Acoustic Scattering Using Convolutional Neural Networks

Acoustic scattering is strongly influenced by boundary geometry of objects over which sound scatters. The present work proposes a method to infer object geometry from scattering features by training convolutional neural networks. The training data is generated from a fast numerical solver developed on CUDA. The complete set of simulations is sampled to generate multiple datasets containing different amounts of channels and diverse image resolutions. The robustness of our approach in response to data degradation is evaluated by comparing the performance of networks trained using the datasets with varying levels of data degradation. The present work has found that the predictions made from our models match ground truth with high accuracy. In addition, accuracy does not degrade when fewer data channels or lower resolutions are used.

==> text/RelatedWork.tex <==
% \vspace{-12pt}
\section{Related Work}
\begin{comment}
In-air sonar systems have been widely used for acoustic imaging \cite{Kerstens2019Mimo,Moebus2007Ultrasound,Steckel2015EmitterArray,Steckel2013Broadband,Strakowski2006PhaseBeamforming}. In these systems, ultrasonic signals are used to ensure specular reflection of acoustic waves. Although these systems are reported to be capable of revealing geometric information of objects such as direction, distance and shape, there are limitations inherent to using ultrasonic signals in these systems. As reported in \cite{Steckel2015EmitterArray}, using ultrasonic signals for long-range sensing is difficult as air is a poor medium for transmission. In addition, the echoes from small objects have minimal acoustic energy, making them hard to be detected even in a middle range. Furthermore, ultrasonic wavelengths are too large for some applications. As a result, reflectors with surfaces at oblique angles to sensor arrays cannot be detected with considerable accuracy.
\end{comment}

In addition, researchers have used indoor acoustic measurements to construct room geometries 
\cite{Antonacci2010Reconstruction,Ba2010L1,Baba2016Multiple,Canclini2011Doa2Loc,Canclini2011Exact,Dokmanic2013NAS,Dokmanic2011RoomShape2D,Filos2012Linear,Filos2010TwoStep,Michael2019Spherical,Moore2013SingleChannel,Naseri2017Cooperative,Nastasia2011Localization,Remaggi2014Room,Remaggi2017Novel,Remaggi20153D,Remaggi2015Source,Tervo20123D}. The existence and uniqueness of mappings from room geometries to in-room acoustic signals were demonstrated in \cite{Dokmanic2013NAS} and \cite{Dokmanic2011RoomShape2D}, serving as the theoretical basis for all related studies. Many different acoustic metrics were used in these studies, such as time of arrival (TOA), direction of arrival (DOA), reverberation and RIR. All of these approaches used apriori mathematical assumptions based on specular reflections, but they used different algorithms to search reflecting planes based on different geometric settings of speaker and microphone arrays. 

Very recently, Lindell et al. proposed a non-line-of-sight (NLOS) acoustic-imaging system capable of constructing the shape of objects behind a wall, using only acoustic measurements \cite{Lindell2019Nlos}. In Lindell's work, sound was assumed to propagate to the hidden object and back to a microphone both through specular reflections at a side wall. Different boundaries of objects for scattering were considered. Reconstructions from both confocal and non-confocal source-receiver settings were analyzed. In addition to the success of recovering letter-shaped objects, the authors also reported failure in detecting objects of weak diffuse components or of surfaces that reflect sound away from the acoustic array.

The present work seeks to build upon the previous work and contribute a new, generalizable approach for estimating room geometries. Our approach differs from the previous approaches in that: (1) We use dense acoustic fields rather than acoustic signals, sampled at several limited receiver locations. As a result, our method utilizes more acoustic features such as diffraction and occlusion, in addition to reflection. (2) We train a CNN to estimate the mapping from acoustic fields to boundary conditions of objects. Thus, our approach is not limited by an analytical model. The only apriori consideration of our approach is the Helmholtz equation. (3) To address the difficulty of acquiring data, we simulate acoustic fields using a high-performance solver. By doing this, our dataset can be generalized to more complex scenarios, e.g., estimation of geometric information of the combination of convex and non-convex objects.
